Two-stage Stochastic Matching and Pricing with Applications to Ride Hailing

Matching and pricing are two critical levers in two-sided marketplaces to connect demand and supply. The platform can produce more efficient matching and pricing decisions by batching the demand requests. We initiate the study of the two-stage stochastic matching problem, with or without pricing, to enable the platform to make improved decisions in a batch with an eye toward the imminent future demand requests. This problem is motivated in part by applications in online marketplaces such as ride hailing platforms. We design online competitive algorithms for vertex-weighted (or unweighted) two-stage stochastic matching for maximizing supply efficiency, and two-stage joint matching and pricing for maximizing market efficiency. In the former problem, using a randomized primal-dual algorithm applied to a family of ``balancing'' convex programs, we obtain the optimal $3/4$ competitive ratio against the optimum offline benchmark. Using a factor revealing program and connections to submodular optimization, we improve this ratio against the optimum online benchmark to $(1-1/e+1/e^2)\approx 0.767$ for the unweighted and $0.761$ for the weighted case. In the latter problem, we design optimal $1/2$-competitive joint pricing and matching algorithm by borrowing ideas from the ex-ante prophet inequality literature. We also show an improved $(1-1/e)$-competitive algorithm for the special case of demand efficiency objective using the correlation gap of submodular functions. Finally, we complement our theoretical study by using DiDi's ride-sharing dataset for Chengdu city and numerically evaluating the performance of our proposed algorithms in practical instances of this problem.

==> new/numerical.tex <==
In this section,
we propose a numerical experiment setup as follows.

\paragraph{Data.}
The main data source in this setup is 
\texttt{TLC Trip Record Data}.\footnote{\url{https://www1.nyc.gov/site/tlc/about/tlc-trip-record-data.page}}
TLC
records include fields capturing pick-up and drop-off dates/times, pick-up and drop-off locations, trip distances, itemized fares, rate types, payment types, and driver-reported passenger counts. The data used in the attached datasets were collected and provided to the NYC Taxi and Limousine Commission (TLC) by technology providers authorized under the Taxicab \& Livery Passenger Enhancement Programs (TPEP/LPEP). 

\paragraph{Two-stage matching instance construction.}
We first cluster all pick-up and drop-off location
in TLC based on their geographical information.
For each cluster, 
we define its demand (resp.\ supply) as 
the number of trips whose pick-up (resp.\ drop-off) 
locations is this cluster.

To construct the driver set $\Driver$, each cluster will be 
selected as a driver 
independently at random 
with probability proportional to its demand.

To construct the rider set $\Rider = \Ra \cup \Rp$,
we first randomly split the supply in each cluster
into two parts (corresponding to 
the first stage and second stage). Each 
cluster will be selected as a rider at 
the first (resp.\ second) stage 
independently at random 
with probability proportional to its supply 
at the first (resp.\ second) stage.

Edge between riders and drivers 
will be randomly generated 
with probability proportional to the distance 
between clusters.

All other parameters (i.e., $\mathbf w, \boldsymbol \pi$)
will be generated in an ad hoc fashion.

\paragraph{Policies}
We implement and compute
the expected performance of \Cref{alg:weighted-skeleton},
\Cref{alg:online}, optimum offline
and myopic greedy (i.e., find a maximum weighted matching in the first stage, 
and then find a maximum weighted matching in the second stage) by 
Monte Carlo method.

==> tex/apx-thm-opt-offline.tex <==
Given \Cref{lemma:structure}, we prove \Cref{thm:opt-offline-comp-ratio} by a randomized primal-dual analysis. 
\optofflinecompratio*
\begin{proof}
We prove the desired competitive ratio against $\optoff$ for \emph{any} realization of $\Rpa$. Fix a realization of $\Rpa$, and consider the linear program of maximum vertex-weighted bipartite matching in $G[\Rpa\cup\Ra, D]$ as the primal LP, and its dual: 
\begin{equation}
\tag{LP-1}
\label{eq:LP-max-weight}
\begin{array}{llllllll}
\max  &\displaystyle\sum_{i\in\Ra\cup\Rpa}\displaystyle\sum_{j\in N(i)}x_{ij}w_j &\text{s.t.}&
&\text{min} &\displaystyle\sum_{i\in \Ra\cup\Rpa }{\alpha_i}+\displaystyle\sum_{j\in D}{\beta_j}&\text{s.t.} \\[1.4em]
 &\displaystyle\sum_{j\in N(i)}{x_{ij}}\leq1 &  i\in\Ra\cup\Rpa~,& 
& &\alpha_i+\beta_j\geq w_j& i\in\Ra\cup\Rpa,j\in N(i)~,\\[1.4em]
 &\displaystyle\sum_{i\in N(j)}{x_{i,j}}\leq 1 &j\in D~, &
& &\alpha_i\geq 0 &i\in \Ra\cup\Rpa~, \\
 &x_{ij} \geq 0 &i\in\Ra\cup\Rpa,j\in N(i)~. &
& &\beta_j\geq 0  &j\in D~. 
\end{array}
\end{equation}
Note that the optimal objective value of the above LP is what $\optoff$ obtains for this particular realization of $\Rpa$. Now let $M_2$ be the maximum vertex-weighted matching between $\Rpa$ and remaining unmatched drivers in $D$ by $M_1$. We construct a randomized dual assignment $\{\alpha_i\},\{\beta_j\}$ for the above dual LP by using matching $M_1$, so that it is feasible in expectation and 
\begin{equation}
\label{eq:primal-dual-ratio}
\expect[M_1]{\sum_{j\in D}w_j\mathbbm{1}\{\textrm{$j$ is matched by $M_1\cup M_2$}\}}= \tfrac{3}{4}\cdot\expect[M_1]{\displaystyle\sum_{i\in \Ra\cup\Rpa }{\alpha_i}+\displaystyle\sum_{j\in D}{\beta_j}}~,
\end{equation}
where $M_1$ is sampled by the randomized rounding step of \Cref{alg:weighted-skeleton} (with marginal edge probabilities $\xbf^*$). This finishes the proof, because $\{\expect{\alpha_i}\},\{\expect{\beta_j}\}$ is a deterministic feasible dual assignment whose objective value is at most $\tfrac{4}{3}$ fraction of the expected weight of the matching $M_1\cup M_2$, and the objective value of any feasible dual assignment is an upper bound on the optimal primal objective value.

Let $D_1$ be the set of matched drivers by $M_1$. Consider the linear program for the maximum vertex-weighted bipartite matching in the residual graph $G[\Rpa, (D\setminus D_1)]$. Let $\{\hat{\alpha}_i\}_{i\in\Rpa}$, $\{\hat\beta_j\}_{j\in D\setminus D_1}$ be the optimal dual solution of this LP. Therefore:
$$\forall i\in\Rpa,j\in D\setminus D_1, (i,j)\in E:~~~\hat\alpha_i+\hat\beta_j\geq w_j$$
Moreover, as $M_2$ is an optimal solution for the primal LP, we have:
$$\sum_{j\in D}w_j\mathbbm{1}\{\textrm{$j$ is matched by $ M_2$}\}=\sum_{i\in\Rpa}\hat\alpha_i+\sum_{j\in D\setminus  D_1}\hat\beta_j$$
Now, given the decomposition in \Cref{lemma:structure}, consider the following randomized dual assignment for \ref{eq:LP-max-weight}:
\begin{itemize}
\item Riders in $\Ra\cup\Rpa:$
\begin{itemize}
    \item $ i\in\Rpa:~~\alpha_i\leftarrow\hat{\alpha}_i$~,
    \item $ i\in \Rider^{(l)},~l=0,1,\dots,L:~\alpha_i\leftarrow c^{(l)}=w_j(1-\sum_{i'\in N(j)}x^*_{i'j}),$ for any driver $j\in\Driver^{(l)}$\\ (\emph{see the uniformity, \Cref{lemma:structure}}).
\end{itemize}
\item Drivers in $D:$
\begin{itemize}
    \item $ j\in \Driver^{(l)},  l=0,1,\dots,L:~~\beta_j\leftarrow w_j\left(\sum_{i\in N(j)}x^*_{ij}\right)^2+\hat\beta_j\mathbbm{1}\{j\in D\setminus D_1\}$~.
\end{itemize}
\end{itemize}
Let $y^*_j\triangleq \sum_{i\in N(j)}x^*_{ij}$ for $j\in D$ denote the probability that $j$ is matched in $M_1$. First, we have:
\begin{align*}
    \sum_{i\in\Ra\cup\Rpa}\alpha_i+\sum_{j\in D}\beta_j&=\sum_{i\in\Ra}\alpha_i+\sum_{j\in D}w_j{y^*_j}^2+\left(\sum_{i\in\Rpa}\hat{\alpha_i}+\sum_{j\in D\setminus D_1}\hat{\beta}_j\right)\\
    &=\sum_{l=0}^{L}\left(\sum_{i\in\Rider^{(l)}}c^{(l)}+\sum_{j\in \Driver^{(l)}}w_j{y^*_j}^2\right)+\sum_{j\in D}w_j\mathbbm{1}\{\textrm{$j$ is matched by $ M_2$}\}\\
    &\overset{(1)}{=}\sum_{l=0}^{L}\left(\sum_{i\in\Rider^{(l)}}\left(\sum_{j\in N(i)}x^*_{ij}\right)c^{(l)}+\sum_{j\in \Driver^{(l)}}w_j{y^*_j}^2\right)+\sum_{j\in D}w_j\mathbbm{1}\{\textrm{$j$ is matched by $ M_2$}\}\\
    &\overset{(2)}{=}\sum_{l=0}^{L}\left(\sum_{i\in\Rider^{(l)}}\sum_{j\in N(i)}x^*_{ij}w_j(1-y^*_j)+\sum_{j\in \Driver^{(l)}}\sum_{i\in N(j)}x^*_{ij}w_j{y^*_j}\right)+\sum_{j\in D}w_j\mathbbm{1}\{\textrm{$j$ is matched by $ M_2$}\}\\
    &=\sum_{l=0}^{L}\sum_{i\in\Rider^{(l)}}\sum_{j\in N(i)}x^*_{ij}w_j+\sum_{j\in D}w_j\mathbbm{1}\{\textrm{$j$ is matched by $ M_2$}\}\\
    &=\sum_{j\in D}w_j\left(\sum_{i\in N(j)}x^*_{ij}+\mathbbm{1}\{\textrm{$j$ is matched by $ M_2$}\}\right)~,
\end{align*}
where (1) holds as either $c^{(l)}=0$ (when $l=0$) or $\sum_{j\in N(i)}x^*_{ij}=1$ (when $l>1$) because of saturation property (\Cref{lemma:structure}), and (2) holds as $c^{(l)}=w_j(1-y^*_j)$ for any $j\in \Driver^{(l)}$ because of uniformity (\Cref{lemma:structure}). Therefore, $\expect[M_1]{ \sum_{i\in\Ra\cup\Rpa}\alpha_i+\sum_{j\in D}\beta_j}=\expect[M_1]{\sum_{j\in D}w_j\mathbbm{1}\{\textrm{$j$ is matched by $ M_1\cup M_2$}\}}$. To check the feasibility, note that the dual constraints in \ref{eq:LP-max-weight} correspond to two types of edges:
\begin{itemize}
    \item $\Big[$\emph{Type \Rom{1}}: $(i,j)\in E, i\in\Ra,j\in D\Big]$ Suppose $i\in\Rider^{(l)}$ and $j\in \Driver^{(l')}$, for $l,l'\in\{0,1,\dots,L\}$. Then:
    $$
    \alpha_i+\beta_j\geq c^{(l)}+w_j{y^*_j}^2\overset{(1)}{\geq}c^{(l')}+w_j{y^*_j}^2\overset{(2)}{=}w_j(1-y^*_j)+w_j{y^*_j}^2\overset{(3)}{\geq} \tfrac{3}{4}w_j~,
    $$
    where (1) and (2) hold because of monotonicity and uniformity properties respectively (\Cref{lemma:structure}), and (3) holds as $y^*_j\in[0,1]$, and $\underset{x\in [0,1]}{\min}1-x+x^2=\tfrac{3}{4}$. Therefore, $\expect[M_1]{\alpha_i+\beta_j}\geq \tfrac{3}{4}w_j$.
     \item $\Big[$\emph{Type \Rom{2}}: $(i,j)\in E, i\in\Rpa,j\in D\Big]$ In this case, we have:
     \begin{align*}
     \expect[M_1]{\alpha_i+\beta_j}&= \expect[M_1]{\hat\alpha_i+w_j{y^*_j}^2+\hat\beta_j\mathbbm{1}\{\textrm{$j$ is not matched in $M_1$}\}}\\
     &=\expect[M_1]{\hat\alpha_i+\hat\beta_j+w_j{y^*_j}^2-\hat\beta_j\mathbbm{1}\{\textrm{$j$ is matched in $M_1$}\}}\\
     &\geq \expect[M_1]{w_j+w_j{y^*_j}^2-\hat\beta_j\mathbbm{1}\{\textrm{$j$ is matched in $M_1$}\}}\\
     &\overset{(1)}{\geq} w_j(1+{y^*_j}^2)-w_j\prob{\textrm{$j$ is matched in $M_1$}}=w_j(1-y^*_j+{y^*_j}^2)\overset{(2)}{\geq}\tfrac{3}{4}w_j~,
    \end{align*}
    where (1) holds as $\hat\beta_j\leq w_j$ (as it is optimal dual solution of the residual LP), and again (2) holds similar to the previous discussion for Type~\Rom{1} edges.
\end{itemize}
Multiplying the current $\{\alpha_i\}$, $\{\beta_j\}$ by $\tfrac{4}{3}$ gives a feasible in expectation dual solution satisfying \Cref{eq:primal-dual-ratio}, which finishes the proof.
\end{proof}

==> tex/further-related-work.tex <==

\paragraph{Two-stage 
stochastic combinatorial optimization}
\citet{KS-06} consider two-stage 
stochastic matching in general graph
where 
the whole graph is fixed across two stages
but 
the edge weights
changes stochastically.
They prove the NP-completeness and design polynomial time policy
which is $\sfrac{1}{2}$-competitive against 
the optimum online policy for matching weights
maximization.
\citet{EGMS-10} improve
\citet{KS-06} results by 
showing APX-hardness and introducing
a new polynomial time policy whose
competitive ratio depends on the maximum degree.
\citet{KKU-08} consider two-stage stochastic
matching in bipartite graph where
the whole graph is fixed but 
the edge costs changes stochastically.
Their goal is to design policy which 
produces perfect (or near perfect) matching
the minimum costs.
They prove NP-hardness and 
polynomial time policy which approximates
the optimum online policy.
Notice that none of these results consider
the same model and are comparable to results in our paper.
Besides matching problem, other 
two-stage stochastic combinatorial optimization
problems have also been considered in the 
literature
% \citep[e.g.][]{BL-11,CCP-05,DST-03,SS-04,SS-07,IKMM-04}.
\citep[c.f.][]{BL-11}.

Our result for the unweighted version of the two-stage matching is closely related to the beautiful work of \cite{LS-17}, which also uses the matching skeleton of \cite{GKK-12}, but for a different two-stage matching problem. In their model, a batch of new edges arrive adversarially in the second stage, and their algorithm first finds a maximum fractional matching using the matching skeleton and then removes some of the edges in the first stage through a randomized procedure to obtains a $\tfrac{2}{3}$-competitive ratio.
 

\paragraph{Online bipartite matching}
Our results for weighted two-stage matching
for supply efficiency (\Cref{sec:matching})
is comparable with results in
\emph{online bipartite matching 
with vertex arrival},
which
studies the competitive ratio against the optimum offline 
in bipartite
matching problem where vertices on one side
arrive in an online fashion. 
For prior-free setting (i.e., no prior for 
online vertices in the future),
\citetalias{KVV-90} design \texttt{Ranking}
which is $(1 - \sfrac{1}{e})$-competitive
for unweighted setting and show it is optimal.
\citet{AGKM-11, DJK-13} generalize 
% the $(1-\sfrac{1}{e})$-competitive 
this result to 
the setting with weighted offline vertices.
\citet{FMMM-09} consider
Bayesian setting with unweighted vertices,
and design a $0.67$-competitive algorithm.
\citet{MGS-12} improve the result
with a $0.702$-competitive algorithm.
 
 


\paragraph{Prophet inequality}
The results in two-stage joint matching/pricing (\Cref{sec:matching and pricing})
is close to some results in
\emph{prophet inequality},
which studies the competitive ratio 
of online algorithms against 
optimum offline in Bayesian selection problem
subject to feasibility constraints.
Two differences between prophet inequality 
and our model are (a) in prophet inequality
algorithms observe 
the value realizations, 
while in our model
algorithms only observe riders' demand (i.e.\ whether
accept their prices) instead of their private
values; (b)
in prophet inequality algorithms 
can be adaptive, while in our model
the prices for riders at 
the second stage need to be determined in advance.
% The first result in prophet inequality by
% \citet{KS-77} show that for 1-uniform matroid,
% there exists $\sfrac{1}{2}$-competitive online algorithm
% against the optimum offline, and the ratio is optimal.
% \citet{KW-12} generalize $\sfrac{1}{2}$-competitive result
% to all matroid environments.
% However, both their algorithms are adaptive (i.e.
% actions on every step depend on the whole history), thus, 
% is not comparable with
% our model where the the prices for riders at 
% the second stage need to be determined in advance.
Therefore, only results for 
algorithms with non-adaptive-thresholds
\footnote{Algorithm fix a non-adaptive threshold for each 
element. Whether elements are selected by the algorithms only depends on whether the value realization is above the threshold.}
in prophet inequality are comparable with our model.
% Fortunately, the literature also considers
% simple (e.g., non-adaptive, symmetric) algorithms in prophet inequality.
For $1$-uniform matroid,
% \footnote{It can be modeled as demand efficiency
% (i.e.\ welfare of riders)
% maximization for instances with a single driver.} 
\citet{sam-84} give a 
$\sfrac{1}{2}$-competitive
non-adaptive algorithm.
For edge-weighted matching with edges arrivals,
% \footnote{It can be modeled as market efficiency
% (i.e.\ welfare of both riders and drivers)
% maximization.} 
\citet{CHMS-10} give a
$\sfrac{4}{27}$-competitive non-adaptive algorithm.
\citet{GW-19} improve the result with a $\sfrac{1}{3}$-competitive non-adaptive
algorithm.
For edge-weighted matching with  
vertices arrivals,
\citet{AHL-12} give a $\sfrac{1}{2}$-competitive
algorithm with non-adaptive-thresholds.
For general matroid environment,
% \footnote{It can be modeled as 
% demand efficiency or supply efficiency maximization.
% }
\citet{FSZ-16} develop the technique so-called online contention resolution
which induces a $\sfrac{1}{4}$-competitive algorithm with non-adaptive-thresholds.
\citet{LS-18} improve the result with a $\sfrac{1}{2}$-competitive
algorithm with non-adaptive-thresholds.

